Denial of Service Attacks on Control Systems with Packet Loss

The performance of control systems with packet loss as a result of an attack over the actuation communication channel is analysed. The operator is assumed to monitor the state of the channel by measuring the average number of packet losses and an attack detection criteria is established based on the statistic. The performance of the attacker is measured in terms of the increase of the linear quadratic cost function of the operator subject to a given detection constraint. Within that setting, the optimal denial of service (DoS) attack strategy is formulated for UDP-like and TCP-like communication protocols. {For both communication protocols,} DoS attack constructions that are independent and identically distributed (IID) are compared to those that are non-stationary. The main contributions of this paper are (i) explicit characterisation of the expected cost increase of the optimal attack constructions and the associated packet loss parameter for the IID case, (ii) proof, by example, that non-stationary random attacks outperform IID attacks in the presence of detection constraints.

==> ifac_ref.tex <==
@article {MPC, 
	author={W. Casbolt and B. Jones and I. Esnaola}, 
	journal={submitted to arXiv}, 
	title={Optimal Control over Multiple Input Lossy Channels}, 
	journal={},
	volume={},
	number={},
	pages={},
	year={2019},
	publisher={}}

%%%%%%%%%%%%%%%%%%%%%%
@ARTICLE{1, 
author={L. {Schenato} and B. {Sinopoli} and M. {Franceschetti} and K. {Poolla} and S. S. {Sastry}},
journal={In Proc. IEEE},
title={Foundations of Control and Estimation Over Lossy Networks},
year={2007},
volume={95},
number={1},
pages={163-187}}
%%%%%%%%%%%%%%%%%%%%
@article{4, 
	author={B. {Sinopoli} and L. {Schenato} and M. {Franceschetti} and K. {Poolla} and S. S. {Sastry}},
	journal={In Proc. American Control Conference},
	title={Optimal control with unreliable communication: the TCP case},
	year={2005},
	volume={5},
	pages={3354-3359}}
%%%%%%%%%%%%%%%%%%%%%%%%%%
@book{6,
	author = {George A. F. Seber},
	title = {A Matrix Handbook for Statisticians},
	year = {2007},
	isbn = {0471748692, 9780471748694},
	edition = {1st},
	publisher = {Wiley-Interscience},
	address = {New York, NY, USA},
} 
%%%%%%%%%%%%%%%%%%
@article{7,
	author = {Bruno Sinopoli and Luca Schenato and Massimo Franceschetti and Kameshwar Poolla and Shankar S. Sastry },
	title = {Optimal linear LQG control over lossy networks without packet acknowledgment},
	journal = {Asian J Control},
	volume = {10},
	number = {1},
	pages = {3-13},
	year = {2008}}
%%%%%%%%%%%%%%%%%%%%%%%%
@article{8, 
	author={Y. {Mo} and E. {Garone} and B. {Sinopoli}},
	journal={European Control Conference (ECC)},
	title={LQG control with Markovian packet loss},
	year={2013},
	volume={},
	number={},
	pages={2380-2385},
	ISSN={}}
%%%%%%%%%%%%%%%%%%%%%%%%%
@ARTICLE{9, 
	author={L. Schenato}, 
	journal={IEEE Transactions on Automatic Control}, 
	title={To Zero or to Hold Control Inputs With Lossy Links?}, 
	year={2009}, 
	volume={54}, 
	number={5}, 
	pages={1093-1099}, 
	keywords={distributed control;linear quadratic control;poles and zeros;stability;hold-input strategy;linear quadratic performance;lossy links;networked control systems;optimal static gain;zero-input strategy;Buffer storage;Communication system control;Control systems;Filters;Intelligent actuators;Networked control systems;Optimal control;Performance gain;Performance loss;Stability;LQ control;networked systems;packet loss;stability}, 
	doi={10.1109/TAC.2008.2010999}, 
	ISSN={0018-9286}, 
	month={May.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@book{SCADA,
	author = {Colbert, E.~J.~M. and Kott, A},
	title = {Cyber-security of SCADA and Other Industrial Control Systems},
	year = {2016},
	isbn = {978-3-319-32123-3, 978-3-319-81203-8},
	publisher = {Springer International Publishing}}


